Towards Efficient Data Valuation Based on the Shapley Value

"How much is my data worth?" is an increasingly common question posed by organizations and individuals alike. An answer to this question could allow, for instance, fairly distributing profits among multiple data contributors and determining prospective compensation when data breaches happen. In this paper, we study the problem of data valuation by utilizing the Shapley value, a popular notion of value which originated in cooperative game theory. The Shapley value defines a unique payoff scheme that satisfies many desiderata for the notion of data value. However, the Shapley value often requires exponential time to compute. To meet this challenge, we propose a repertoire of efficient algorithms for approximating the Shapley value. We also demonstrate the value of each training instance for various benchmark datasets.

==> proof_knn.tex <==
% In the following we first present the pseudocode for the K-NN-based approach of Section \ref{subsec:KNN}.
We introduce two basic lemmas and proceed to the proof of our main result, the recursive K-NN Shapley value computation described in Theorem~\ref{thm:KNN_shaplay}. 
%\dan{Again, previously $*$ meant test. The parentheses on line 5 are needless.}


% \begin{algorithm}[H]
% % \scriptsize
% \caption{K-NN-based Shapley value calculation}
% \label{alg:knn}
%     \hspace*{\algorithmicindent} \textbf{Input:} $D = \{(x_i,y_i)\}_{i=1}^N$ - training set, $D^* = \{(x_\text{test}_i,y_\text{test}_i)\}_{i=1}^{N_{test}}$ - test set, $d(\cdot,\cdot)$ - distance metric \\
%  \hspace*{\algorithmicindent} \textbf{Output:} $\{s_i\}_{i=1}^N$ - Shapley values %, $\{\alpha_i\}_{k=1,...,K} \subseteq I$ - indices of sorted data
%     \begin{algorithmic}[1]
%         \State Initialize $s_{i}\leftarrow 0$ for $i=1,...,N$
%         \For{$i=1$ to $N_{test}$} % $\%$ over test points
%             \State  $(\alpha_1,...,\alpha_N) \leftarrow$ Indices of data in an ascending order using $d(\cdot,x_i^*)$ %\text{FindIncreasingOrder}(d(\cdot,D_i^*), D)$
%             \For{$k=N-1$ to $1$ } %$\%$ recursive average SV calculation over training points
%                 \State $s_{\alpha_k} \leftarrow \left( s_{\alpha_{k+1}} + \frac{\mathbbm{1}[y_{\alpha_k} = y_\text{test}_i]-\mathbbm{1}[y_{\alpha_{k+1}} = y_\text{test}_i]}{K} \frac{\min(K-1, k -1) + 1}{k} \right)$
%             \EndFor
%         \EndFor
%       %\State \fh{Note that $s[\alpha_N]$ is initialized with 0 before the test-point-loop and $s[\alpha_N]$ is not updated within the training point loop, which is equivalent to adding 0 . }
%     \end{algorithmic}
% \end{algorithm}






%\begin{wrapfigure}{r}{0.67\textwidth}
%\vspace{-2em}
%\begin{minipage}{0.67\textwidth}

%\end{minipage}
%\end{wrapfigure}
 %\begin{wrapfigure}{r}{0.5\textwidth}
%\vspace{-4em}
%\begin{minipage}{0.5\textwidth}
%\begin{algorithm}[H]
%\scriptsize
%\caption{Shapley Value for K-NN Classifier}
%\label{alg:knn}
%    \hspace*{\algorithmicindent} \textbf{Input:} $D = \{(x_i,y_i)\}_{i=1}^N$ - training set, $D^* = \{(x_\text{test}_i,y_\text{test}_i)\}_{i=1}^{N_{test}}$ - test set, $d(\cdot,\cdot)$ - distance metric \\
% \hspace*{\algorithmicindent} \textbf{Output:} $\{s_i\}_{i=1}^N$ - Shapley values %, $\{\alpha_i\}_{k=1,...,K} \subseteq I$ - indices of sorted data
%    \begin{algorithmic}[1]
%        \State Initialize $s_{i}\leftarrow 0$ for $i=1,...,N$
%        \For{$i=1$ to $N_{test}$} % $\%$ over test points
%            \State  $(\alpha_1,...,\alpha_N) \leftarrow$ Indices of data in an ascending order using $d(\cdot,\cdot)$ %\text{FindIncreasingOrder}(d(\cdot,D_i^*), D)$
%            \For{$k=N-1$ to $1$ } %$\%$ recursive average SV calculation over training points
%                \State $s_{\alpha_k} \leftarrow s_{\alpha_k} + \frac{1}{N_{test}} \times$
%                \State $~~~~~~~~~~\left( s_{\alpha_{k+1}} + \frac{\mathbbm{1}[y_{\alpha_k} == y_\text{test}_i]-\mathbbm{1}[y_{\alpha_{k+1}} == y_\text{test}_i]}{K} \frac{\min(K-1, k -1) + 1}{k} \right)$
%            \EndFor
%        \EndFor
%       %\State \fh{Note that $s[\alpha_N]$ is initialized with 0 before the test-point-loop and $s[\alpha_N]$ is not updated within the training point loop, which is equivalent to adding 0 . }
%    \end{algorithmic}
%\end{algorithm}
%\end{minipage}
%\end{wrapfigure}


%The following Lemma was used in the proof of Theorem \ref{thm:KNN_shaplay}:

\begin{Lm}
\label{lem:pascal}
% We claim that 
\begin{align}
\label{aux_lemma_knn}
 \sum_{i=0}^{min(a, N)} \sum_{j=0}^{M} \frac{\binom{N}{i}\binom{M}{j}}{\binom{N+M}{i+j}} = (min(a, N)+1)\frac{M+N+1}{N+1}.  
\end{align}
% where $ \binom{N}{i} := \frac{N!}{i! (N-i)!}$ is the binomial coefficient.
\end{Lm}

% \begin{proof}
% \ref{aux_lemma_knn} can be re-written as
% \begin{align}
% \sum_{i=0}^{min(a, N)} \sum_{j=0}^{M} C_N^i C_M^j / C_{N+M}^{i+j} =
% 1/C_{M+N}^M \sum_{i=0}^{min(a, N)} \sum_{j=0}^{M} C_{i+j}^i C_{M+N-i-j}^{N-i}
% \end{align}
% Consider the inner summation $\sum_{j=0}^{M} C_{i+j}^i C_{M+N-i-j}^{N-i}$. First, we show that
% \[
% \sum_{j=0}^{M} C_{i+j}^i C_{M+N-i-j}^{N-i} = C_{M+N+1}^M.
% \]
% Merves intuition was the following. Due to binomial theorem together with exponent combination laws, $\sum_{j=0}^{M} C_{i+j}^i C_{M+N-i-j}^{N-i}$ should be of the coefficient of $x^{M}$ in the expansion of $(1+x)^{N+M+constant}$. Also, there is a much simpler proof using purely Pascal's rule, that is, $C_{M+N+1}^{N+1} = \sum_{k=0}^M C_{M+N-k}^N$, I will add it here too
% Applying Pascal's identity to $C_{M+N+1}^M$ {\it i+1} times in an iterative fashion, we have
% \begin{align}\label{first_pascal_app}
%   C_{M+N+1}^M = \sum_{k=0}^{M} C_{i+1}^{k} C_{M+N-i}^{M-k}. 
% \end{align}
% Further expansion with Pascal's identity implies that
% \begin{align}\label{second_pascal_app}
% C_{M+N-i}^{M-k} =  \sum_{j=k}^M C_{j-1}^{k-1} C_{M+N-i-j}^{M-j}.
% \end{align}
% That is, applying Pascal's identity iteratively to the terms of the form $C_{M+N-i}^{M-k}$, the number of $C_{M+N-i-j}^{M-j}$ terms in this expansion is exactly $C_{j-1}^{k-1}$ where $j\geq k$ by Pascal's rule. Substituting~\ref{second_pascal_app} into~\ref{first_pascal_app}, we have
% \begin{align}
%     C_{M+N+1}^M &= \sum_{k=0}^{M} C_{i+1}^k \sum_{j=k}^{M} C_{j-1}^{k-1} C_{M+N-i-j}^{M-j}\\
%     &=\sum_{j=0}^M \sum_{k=0}^j C_{i+1}^k C_{j-1}^{k-1} C_{M+N-i-j}^{M-j}.
% \end{align}
% Using Chu-Vandermonde identity, we further have $\sum_{k=0}^j C_{i+1}^k C_{j-1}^{k-1} = C_{i+j}^j$. Thus
% \begin{align}\label{inner_term_aux_knn}
%     C_{M+N+1}^M =\sum_{j=0}^M C_{i+j}^j C_{M+N-i-j}^{M-j}.
% \end{align}
% \end{proof}
\begin{proof}[Proof of Lemma \ref{lem:pascal}]
Remark that Equation \ref{aux_lemma_knn} can be re-written as
\begin{align}
\sum_{i=0}^{min(a, N)} \sum_{j=0}^{M} \frac{\binom{N}{i} \binom{M}{j}}{\binom{N+M}{i+j}} =
\frac{1}{\binom{M+N}{M}} \sum_{i=0}^{min(a, N)} \sum_{j=0}^{M} \binom{i+j}{i}\binom{M+N-i-j}{N-i} \, .
\end{align}
 Consider the inner summation $\sum_{j=0}^{M} \binom{i+j}{i} \binom{M+N-i-j}{N-i}$. First, we show that
 \[
 \binom{M+N+1}{N+1} = \sum_{j=0}^{M} \binom{i+j}{i} \binom{M+N-i-j}{N-i}.
 \]
%\mrv{For your taste: My intuition was the following. Due to binomial theorem together with exponent combination laws, $\sum_{j=0}^{M} C_{i+j}^i C_{M+N-i-j}^{N-i}$ should be of the coefficient of $x^{M}$ in the expansion of $(1+x)^{N+M+constant}$.}
A direct application of Hockey-Stick Identity to $\binom{M+N+1}{N+1}$ implies 
\begin{align}\label{hockey_stick}
    \binom{M+N+1}{N+1}=\sum_{i=N}^{M+N} \binom{i}{N}.
\end{align}
Let $k \coloneqq M+N-i$. Equation~\ref{hockey_stick} then becomes
\begin{align}\label{hockey_stick_ourcase}
    \binom{M+N+1}{N+1}=\sum_{k=0}^{M} \binom{M+N-k}{N}.
\end{align}
Next, we apply the above expansion recursively $i+1$ times, that is,
\begin{align}\label{aux_lemma_knn2}
 \binom{M+N+1}{N+1} = \underset{s. t. \  0\leq k_l \leq M-\sum_{m=1}^{l-1} k_m}{\sum_{k_l, \ l\in\{1, 2, \cdots, i+1\}}} \binom{M+N-i-\sum_{l=1}^{i+1}k_l}{N-i}.
\end{align}
Let $j \coloneqq \sum_{l=1}^{i+1}k_l$. We have
\begin{align}\label{aux_lemma_knn3}
 \underset{s. t. \  0\leq k_l \leq M-\sum_{m=1}^{l-1} k_m}{\sum_{k_l, \ l\in\{1, 2, \cdots, i+1\}}} \binom{M+N-i-\sum_{l=1}^{i+1}k_l}{N-i} = \sum_{j=0}^M c_j \binom{M+N-i-j}{N-i}.
\end{align}
% \dan{Why use $\equiv$?}

% The coefficient of each term of the form $\binom{M+N-i-\sum_{l=1}^{i+1}k_l}{N-i}$ hence $\binom{M+N-i-j}{N-i}$ with $j=\{0, 1, \cdots, M\}$ is induced by all different combinations of $k_l$'s, $l=\{ 1, 2, \cdots i+1\}$ such that $\sum_{l=1}^{i+1} k_l = j$.
% %$0\leqk_l\leq M-\sum_{m=1}^{l-1} k_m$. 
The coefficient $c_j$ of each term of the form $\binom{M+N-i-j}{N-i}$ with $j=\{0, 1, \ldots, M\}$ is induced by all different combinations of $k_l$'s, $l\in\{ 1, 2, \cdots i+1\}$ such that $\sum_{l=1}^{i+1} k_l = j$.
%$0\leqk_l\leq M-\sum_{m=1}^{l-1} k_m$. 
Evidently, this is a problem of distributing a total of $j$ indistinguishable numbers to $i+1$ distinguishable summations. Distinguishability is due to the relation that $k_l \leq M-\sum_{m=1}^{l-1} k_m$. A direct application of balls-and-urns (also known as stars-and-bars) implies that the total number of $\binom{M+N-i-j}{N-i}$ terms coming from all different combinations of $k_l$'s with $\sum_{l=1}^{i+1}k_l=j$ is given by $\binom{i+j}{j}$. Hence
%\ref{aux_lemma_knn2} can be re-written as
\begin{align}
 \binom{M+N+1}{N+1} = \sum_{j=0}^M \binom{i+j}{j} \binom{M+N-i-j}{N-i}.
\end{align}
\end{proof}


The following lemma says that the difference in the utility gain induced by either point $i$ or point $j$ translates linearly to the difference in the respective Shapley values, which can be calculated simply by consideration of all possible subsets excluding these points. 

\begin{Lm}
\label{lm:shapley_diff} 
For any $i,j\in I$ and $i\neq j$, the difference in Shapley values between $i$ and $j$ is 
\begin{align}
\label{eqn:shapley_diff}
     s_i-s_j = \frac{1}{N-1}  \sum_{S\subseteq I\setminus\{i,j\}} \frac{1}{\binom{N-2}{|S|}}\big[U(S\cup\{i\}) - U(S\cup \{j\})\big]
\end{align}
\end{Lm}


\begin{proof}
\begin{align}
 s_i-s_j &= \sum_{S\subseteq I\setminus\{i\}} \frac{|S|!(N-|S|-1)!}{N!} \big[U(S\cup \{i\})-U(S)\big] \nonumber\\
 &\quad\quad- \sum_{S\subseteq I\setminus\{j\}} \frac{|S|!(N-|S|-1)!}{N!} \big[U(S\cup \{j\})-U(S)\big]   \\
 &=\sum_{S\subseteq I\setminus\{i,j\}} \frac{|S|!(N-|S|-1)!}{N!} \big[U(S\cup\{i\}) - U(S\cup \{j\})\big] \nonumber\\
 &\quad\quad+\sum_{S\in\{T|T\subseteq I,i\notin T, j\in T\}}  \frac{|S|!(N-|S|-1)!}{N!}   \big[U(S\cup \{i\})-U(S)\big]\nonumber \\
 &\quad\quad-\sum_{S\in\{T|T\subseteq I,i\in T, j\notin T\}} \frac{|S|!(N-|S|-1)!}{N!} \big[U(S\cup \{j\})-U(S)\big]\\
 &=\sum_{S\subseteq I\setminus\{i,j\}} \frac{|S|!(N-|S|-1)!}{N!} \big[U(S\cup\{i\}) - U(S\cup \{j\})\big] \nonumber\\
 &\quad\quad+ \sum_{S'\subseteq I\setminus\{i,j\}} \frac{(|S'|+1)!(N-|S'|-2)!}{N!} \big[U(S'\cup\{i\}) - U(S'\cup \{j\})\big]\\
 &= \sum_{S\subseteq I\setminus\{i,j\}} \big( \frac{|S|!(N-|S|-1)!}{N!} + \frac{(|S|+1)!(N-|S|-2)!}{N!}\big) \nonumber\\
 &\quad\quad\cdot \big[U(S\cup\{i\}) - U(S\cup \{j\})\big]\\
 &=\frac{1}{N-1}  \sum_{S\subseteq I\setminus\{i,j\}} \frac{1}{C_{N-2}^{|S|}}\big[U(S\cup\{i\}) - U(S\cup \{j\})\big] \, .
\end{align}
\end{proof}

Loosely speaking, the proof distinguishes subsets $S$ which include neither $i$ nor $j$ (such that the subset utility $U(S)$ of the marginal contribution directly cancels) and subsets including either $i$ or $j$. In the latter case, $S$ can be partitioned to a mock subset $S'$ by excluding the
% $j^{\text{th}}$ point from $S \subseteq I\setminus \{i\}$ (and vice versa for point $j$),
respective point from S such that a common sum over $S'$ again eliminates all terms other than $U(S' \cup \{i\}) -  U(S' \cup \{j\})$.

In the following we restate, comment and prove Theorem~\ref{thm:KNN_shaplay}. 
\newline
\begin{Thmn}[\ref{thm:KNN_shaplay}] 
Let $x_{\alpha_i}$, $i=1,\ldots,N$, be the training point that is $i$th closest to a given test point $x_\text{test}$. If $K$NN ($K<N$) is used as the classifier and the utility is $U(S) = \frac{1}{K} \sum_{ \alpha_i \in S,i=1,\cdots,\min\{|S|,K\}} \mathbbm{I}[y_{\alpha_i} = y_\text{test}]$, then the Shapley value of each training point can be calculated recursively as follows:
% {\scriptsize
\begin{align}
\label{eqn:recursive_KNN}
&s_{\alpha_N}=\frac{\mathbb{I}[y_{\alpha_{N}} = y_\text{test}]}{N}
\\
& s_{\alpha_i} = s_{\alpha_{i+1}} +  \frac{\mathbb{I}[y_{\alpha_i} = y_\text{test}] - \mathbb{I}[y_{\alpha_{i+1}} = y_\text{test}]}{K}
    \frac{(\min(K-1, i-1) + 1)}{i}.
\end{align}
\end{Thmn}




%\label{thm:KNN_shaplay}

% $\textbf{Theorem}$ \ref{thm:KNN_shaplay} : Let $x_{\alpha_i}$, $i=1,\cdots,N$, be the training point that is $i$th closest to a given test point $x_\text{test}$. If K-NN ($K<N$) is used as the classifier and the utility 
% is $U(S) = \frac{1}{K} \sum_{i : \alpha_i \in S}^{K} \mathbbm{I}[y_{\alpha_i} = y_\text{test}]$, then the Shapley value of each training point can be calculated recursively as follows:
% \begin{align}
% \label{eqn:recursive_KNN}
%  s_{\alpha_N}=0; ~~~ s_{\alpha_i} = s_{\alpha_{i+1}} +  \frac{\mathbb{I}[y_{\alpha_i} = y_\text{test}] - \mathbb{I}[y_{\alpha_{i+1}} = y_\text{test}]}{K}
%     \frac{(\min(K-1, i-1) + 1)}{i}
% \end{align}



The proof is motivated by the following insight:
Recall that the probability $P[x_\text{test} \rightarrow y_\text{test} | S]$ of a correct test label assignment is calculated from the labels of the $K$ points $\alpha_1,..,\alpha_K$ closest to $x_\text{test}$, measured by a given distance $d(\cdot, x_\text{test})$. Recall also that this defines the subset utility $U(S) := \frac{1}{K} \sum_{ \alpha_i \in S,i=1,\cdots,K} \mathbbm{I}[y_{\alpha_i} = y_\text{test}]$, from which we can directly see that $U(S)$ depends only on the K points $\{ x_{\alpha_1}, ..., x_{\alpha_K} \} \subseteq S$ nearest to the test point $x_\text{test}$. 

If we consider the utility $U(S \cup \{i\})$ of the union of $S$ with any point $i$, the K nearest points $ \{ \alpha_1, ..., \alpha_K \} \subseteq S $ within S may not be identical to the K nearest points of the union, that is, $U(S) \neq U(S \cup \{i\})$. 
Adding a point $i$ to a subset changes the utility if and only if the $i$th point is closer to the test point than point $\alpha_{K}$, or, equivalently 
\begin{equation*}
    U(S) = U(S \cup \{i\}) \Longleftrightarrow d(x_{\alpha_K}, x_\text{test}) < d(x_{i},x_\text{test}) \,.
\end{equation*}

This motivates a case distinction if we are interested in the difference in utility $\Delta U(S,i,j) = U(S \cup \{i\}) - U(S \cup \{j\}) $. Following the intuition outlined in Section \ref{subsec:KNN} we now provide a more technical case distinction for the general K-NN-based approach to computing the Shapley value.

%\paragraph*{Intuition of Proof for $K=1$.}
%\fh{ Temporary:  Given an ordered list of training data points
%and one test data point, we
%analyze the difference in utility between two 
%{\em neighboring} training data points. Consider Case 1, where two data points $i$ %and $j$
%have different labels $y_i \neq y_j$. If there is no data point in $S \subseteq I \setminus \{i, j\}$
%that ranks higher (is more similar) than $i$ and $j$ (Case 1.1) then
%the utility difference $\Delta U(S,i,j)$ will be either -1 or 1
%(because $i$ and $j$ will be used by
%the 1-NN algorithm to make a prediction);
%However, if the subset $S$ contains a point $k$ ranked higher than $i$ or $j$ (Case 1.2) then the utility difference $\Delta U(S,i,j)$ 
%will be 0 (because neither $i$ nor $j$, but only $k$, will be used for prediction, hence $U(S \cup \{i\}) = U(S) = U(S \cup \{j\}) $). As we can see, if $i$ and $j$ have identical labels (case 2), the utility difference is 0 for any $S$. Therefore, we can
%simply calculate the Shapley value difference 
%between $i$ and $j$ by counting 
%how many subsets $S$ fall into Case 1.1 and Case 1.2.
%}


\begin{proof}[Proof of Theorem \ref{thm:KNN_shaplay}]

%Given a distance measure  $d(\cdot, \cdot)$, we can sort $(x_1, ..., x_N)$ such that $(\alpha_1,...,\alpha_N)$ are the indices of $x_1, ..., x_N$ ordered by increasing distance $d(\cdot, x_\text{test})$, that is, $x_{\alpha_i}$, $i=1,\cdots,N$, is the training point that is $i$th closest to a given test point $x_\text{test}$.
Let $x_\text{test} \in \mathbb{R}^d$ be the testing point which defines the utility function $U(S) := \frac{1}{K} \sum_{ \alpha_i \in S,i=1,\cdots,K} \mathbbm{I}[y_{\alpha_i} = y_\text{test}]$ for a K-NN classifier with training points $\{x_{\alpha_i}\}_{i=1}^N$ and labels $\{y_{\alpha_i}\}_{i=1}^N$. Let  $d(\cdot, \cdot) : \mathbb{R}^d \times \mathbb{R}^d \rightarrow \mathbb{R}$ be the distance measure according to which $\{\alpha_i\}_{i=1}^{N}$ is determined. 


W.l.o.g., we
assume that $x_1,\ldots, x_n$ are
sorted according to their similarity $d(\cdot, x_\text{test})$
with $x_\text{test}$, that is, $x_i = x_{\alpha_i}$ 
 ($x_1$ is most
similar to $x_\text{test}$). We further assume
that there are no ties in terms of similarity.
This procedure can be finished by
$Nd + N \log N$ operations
where $d$ is the dimension of features.


%\end{Lem}

%\begin{align}
%    s_i - s_{i+1} 
%    &=\frac{1}{N-1} \sum_{k=0}^{N-2} \frac{1}{C_{N-2}^{k}} \sum_{S\subseteq I\setminus\{i,i+1\},|S|=k}\bigg[U(S\cup\{i\}) - U(S\cup \{i+1\})\bigg]
%\end{align}

We now choose to split a subset $S\subseteq I\setminus\{i,i+1\}$ of size $k$ into two disjoint sets $S_1$ and $S_2$ with $S = S_1 \cup S_2$ and  $|S_1| + |S_2| = |S| = k $. Given two neighboring points with indices $i,i+1 \in I$ we constrain $S_1$ and $S_2$ to $S_1 \subseteq \{1,...,i-1\}$
and $S_2 \subseteq \{i+2,...,N\}$. 

Let $s_i$ be the Shapley value of data point $x_i$.
Recall from Lemma \ref{lm:shapley_diff} that for any $i,j\in I$ and $i\neq j$, the difference of Shapley values between $i$ and $j$ is
% {\scriptsize
\begin{align}
\label{eqn:shapley_diff}
     s_i-s_j = \frac{1}{N-1}  \sum_{S\subseteq I\setminus\{i,j\}} \frac{1}{\binom{N-2}{|S|}}\big[U(S\cup\{i\}) - U(S\cup \{j\})\big]
\end{align}
% }

We can now draw conclusions about the utility function $U(S \cup \{i\})$ of any subset $S \subseteq I\setminus\{i,i+1\}$ and the resulting Shapley value by considering the following cases: 


\paragraph{Case 1.1}
Consider the case $|S_1| < K$ with $y_i \neq y_{i+1}$. We then know that $i < K$ and therefore $U(S \cup \{i\}) \neq U(S)$ if $y_i \neq y_{i+1}$. However, the difference of 
including a point $i$  affects only one term in the sum $U(S) := \frac{1}{K} \sum_{k \in S}^{K} \mathbbm{I}[y_{\alpha_k} = y_\text{test}]$ over all K nearest neighbors, i.e.
\begin{align}
    U(S\cup\{i\}) - U(S) = \left\{\begin{array}{l}
         \frac{1}{K}( \mathbbm{I}[y_{i} = y_\text{test}] - \mathbbm{I}[y_{K} = y_\text{test}] ) \quad \text{when $|S|\geq K$} \\
         \frac{1}{K}\mathbbm{I}[y_{i} = y_\text{test}] \quad \text{when $|S|< K$}
    \end{array}
    \right.
\end{align}
The same holds for the inclusion of point $i+1$. 
Therefore,
\[
U(S\cup\{i\}) - U(S\cup \{i+1\}) = 
    \frac{\mathbb{I}[y_i = y_\text{test}] - \mathbb{I}[y_{i+1} = y_\text{test}]}{K}
\]

Using (\ref{eqn:shapley_diff}) we have
\begin{align}
    s_i - s_{i+1}
    &=\frac{1}{N-1} \sum_{k=0}^{N-2} \frac{1}{\binom{N-2}{k}} 
     \sum \limits_{ \substack{  S_1 \subseteq \{1,...,i-1\}, \\ S_2 \subseteq \{i+2,...,N\}: \\ |S_1| + |S_2|=k, |S_1| < K} }
       \frac{\mathbb{I}[y_i = y_\text{test}] - \mathbb{I}[y_{i+1} = y_\text{test}]}{K} \, .
\end{align}

\paragraph{Case 1.2}
Consider the case $|S_1| \geq K$ with $y_i \neq y_{i+1}$. We then know that $i > K$ and therefore $U(S \cup \{i\}) = U(S)$, hence the term  $U(S\cup\{i\}) - U(S)$ is zero. Since the same holds for point $i+1$ ($i+1 \geq K$ and  $U(S \cup \{i+1\}) = U(S)$) and by (\ref{eqn:shapley_diff}), it follows that
\begin{align}
    s_i - s_{i+1} 
    &=\frac{1}{N-1} \sum_{k=0}^{N-2} \frac{1}{\binom{N-2}{k}} 
     \sum \limits_{ \substack{  S_1 \subseteq \{1,...,i-1\}, \\ S_2 \subseteq \{i+2,...,N\}: \\ |S_1| + |S_2|=k, |S_1| \geq K} } \bigg[U(S\cup\{i\}) - U(S\cup \{i+1\})\bigg] = 0 \, .
\end{align}

\paragraph{Case 2} Consider the case of neighboring training points with identical labels $y_i = y_{i+1}$. From $\mathbbm{I}[y_{i} = y_\text{test}] = \mathbbm{I}[y_{i+1} = y_\text{test}]$ and $U(S)= \frac{1}{K} \sum_{k \in S}^{K} \mathbbm{I}[y_{\alpha_k} = y_\text{test}]$ we directly conclude $U(S \cup \{i\}) = U(S \cup \{i+1\})$  for any $S\subseteq I\setminus \{i, i+1\}$ and therefore $s_i - s_{i+1} = 0 $.

\paragraph{Rewriting the Non-Trivial Shapley Difference}
In the following we consider only the non-trivial case (Case 1.2).
Note that $\frac{\mathbb{I}[y_i = y_\text{test}] - \mathbb{I}[y_{i+1} = y_\text{test}]}{K}$ does not depend on the summation at all:
\begin{align}
\begin{aligned}
    s_i - s_{i+1} 
    &=
    \frac{\mathbb{I}[y_i = y_\text{test}] - \mathbb{I}[y_{i+1} = y_\text{test}]}{K}
    \times
    \frac{1}{N-1} \sum_{k=0}^{N-2} \frac{1}{\binom{N-2}{k}}
    \sum \limits_{ \substack{  S_1 \subseteq \{1,...,i-1\}, \\ S_2 \subseteq \{i+2,...,N\}: \\ |S_1| + |S_2|=k, |S_1| < K} } 1 \\
    &=
    \frac{\mathbb{I}[y_i = y_\text{test}] - \mathbb{I}[y_{i+1} = y_\text{test}]}{K}
    \times
    \frac{1}{N-1} \sum_{k=0}^{N-2} \frac{1}{\binom{N-2}{k}} 
    \sum_{m = 0}^{\min(K-1,k)} \binom{i-1}{m}  \binom{N-i-1}{k-m}
    \end{aligned}
\end{align}
%\paragraph*{Result for $\kappa$-NN} 
Then, we can use Lemma \ref{lem:pascal} to analyze the following term:
\begin{align}
\sum_{k=0}^{N-2} \frac{1}{\binom{N-2}{k}} 
    \sum_{m = 0}^{\min(K-1,k)} \binom{i-1}{m} \binom{N-i-1}{k-m} 
= &
\sum_{m=0}^{\min(K-1, i-1)} \sum_{k'=0}^{N-i-1} \frac{\binom{i-1}{m} \binom{N-i-1}{k'}}   {\binom{N-2}{m+k'}} 
\end{align}

Take $i-1=N$ and $N-i-1=M$ in Lemma \ref{lem:pascal} to get
\begin{align}
\sum_{k=0}^{N-2} \frac{1}{\binom{N-2}{k}} 
    \sum_{m = 0}^{\min(K-1,k)} \binom{i-1}{m} \binom{N-i-1}{k-m}  = \frac{ (\min(K-1, i-1) + 1)}{i}
    (N-1)  
\end{align}
Therefore, we have the following recursion
\begin{align}
    s_i - s_{i+1} =
\frac{\mathbb{I}[y_i = y_\text{test}] - \mathbb{I}[y_{i+1} = y_\text{test}]}{K}
    \frac{(\min(K-1, i-1) + 1)}{i}
\end{align}

Now, we analyze the formula for $s_N$, the starting point of the recursion. Since $x_N$ is farthest to $x_\text{test}$ among all training points, $x_N$ results in non-zero marginal utility only when it is added to a set of size smaller than $K$. Hence, $s_N$ can be written as
\begin{align}
    s_N &= \frac{1}{N} \sum_{k=0}^{K-1} \frac{1}{{N-1\choose k}} \sum_{|S|=k, S\subseteq I\setminus\{N\}} U(S\cup N) - U(S)\\
    &=\frac{1}{N}\sum_{k=0}^{K-1} \frac{1}{{N-1\choose k}} \sum_{|S|=k, S\subseteq I\setminus\{N\}} \frac{\mathbb{I}[y_N=y_\text{test}]}{K}\\
    &= \frac{\mathbb{I}[y_N=y_\text{test}]}{N}
\end{align}
\end{proof}



==> pseudo_code_gt.tex <==
We provide the implementation of the group testing-based approach in Algorithm~\ref{alg:gt}. 

\begin{algorithm}[h]
% \scriptsize
\caption{Group-Testing-Based Shapley Value approximation}
\label{alg:gt}
    % \hspace*{\algorithmicindent} 
    \textbf{Input: } $D=\{z_i\}_{i=1}^N$ - training dataset, $U(\cdot) \in [0,r]$ - utility function, $\epsilon,\delta$ - approximation error parameters\\
%  \hspace*{\algorithmicindent} 
\textbf{Output: } $(\hat{s}_1 , ... \hat{s}_N)$  - estimated Shapley values\\
%  \hspace*{\algorithmicindent}
\textbf{Variables: } $Z$ - Normalization constant, $T$ -  number of tests , $\epsilon$ - error bound,  $A \in \{0,1\}^{T \times N}$ -  activation matrix, $B\in [0,r]^{T}$ - utility matrix, $C_{ij}$ - estimated Shapley value difference between $i$ and $j$ where $i,j\in \{1,\cdots,N\}$
%test matrix (average testing difference between users i and j)
 
    \begin{algorithmic}[1]
        % \State Choose $\epsilon < \frac{1}{N} $
        
        \State $U_{tot} \leftarrow U(D)$ 
        
        \State  $Z \leftarrow 2\sum _{k=1}^{N-1} \frac{1}{k}$
        
       % \State $T \leftarrow \frac{1}{\epsilon^2} 2 r^2 Z^2 \log(\frac{N (N-1)}{\delta}) $ 
        %($T \leftarrow \text{ GetNumberOfTests}(\epsilon, \delta)$)
        \State $q(k)\leftarrow\frac{1}{k} (\frac{1}{k} + \frac{1}{N-k})$ for $k=1,\cdots,N-1$
        \State  $q_{tot} \leftarrow \frac{N-2}{N}q(1) + \sum_{k=2}^{N-1} q(k)\big[1+\frac{2k(k-N)}{N(N-1)}\big]$ 
        \State $T\leftarrow \frac{4}{(1-q_{tot}^2)h\big(\frac{2\epsilon}{ZrC_{\epsilon}(1-q_{tot}^2)}\big)} \log \frac{C_{\delta}(N-1)}{2\delta}$
        %  \State $T \leftarrow  \frac{4}{(1-q_{tot}^2)h(\frac{2\epsilon}{Zr(1-q_{tot}^2)})} \log \frac{N(N-1)}{2\delta}$, where $h(u)=(1+u)\log(1+u) - u$
        \State Initialize $(a)_{ti} \leftarrow 0$, $t= 1, ..., T, i = 1,..., N $
        
        \For{$t = 1$ to $T$}
            \State Draw $k_t \sim q(k)$
            %\State $O(N,k) \leftarrow \text{GenerateUniformRandomPermutation}(N,k)$
            %\State Draw $ a_{ti} \sim \text{Ber}( \frac{1}{C^{k_t}_{N}})$ for $i=1,..,N$ while $\sum_{i=1}^{N} a_{ti} < k $
            
            \For{$j=1$ to $k_t$} 
                \State Uniformly sample a length-$k_t$ sequence $I_{j}$ from $\{1,\cdots,N\}$ 
                %${N\choose k}$ all possible length-$k$ sequences
                %index(iter)  $ \sim  \frac{1}{N}$
                \State $a_{ti} \leftarrow 1$ for all $i\in I_j$
            \EndFor
            
            \State $B_t \leftarrow U(\{i : a_{ti} = 1\})$
            
           
        \EndFor
     \State $C_{ij} \leftarrow \frac{Z}{T} \sum_{t=1}^T B_t (A_{ti}- A_{tj})$ for $i = 1,..,N$, $j = 1,...,N$ and $j\geq i$  
    \State Recovering the Shapley value from the estimated Shapley differences $C_{ij}$
    % \State \textbf{Feasibility-based approach to recovering the Shapley value from the Shapley differences:}
    % \State $(s_1,..,s_n) \leftarrow \text{SolveFeasibilityProblem}(C,U_{tot}, N, \epsilon)  $
    \end{algorithmic}
\end{algorithm}

To recover the Shapley value of individual
data points from the estimated 
difference between two data points, there are two
possible approaches. 
\paragraph*{Approach 1: Baseline Points}
The first approach is rather simple: First, we take an arbitrary data point $x_*$,
which we call a ``baseline point'', and estimate its Shapley value $s_*$ up to $(\frac{(C_\epsilon-1)\epsilon}{C_\epsilon},\frac{(C_\delta-1)\delta}{C_\delta})$
 (where $C_\epsilon,C_\delta > 1$)
using the standard sampling-based approach described in Algorithm \ref{alg:sampling}. Then,
for each data point $x_i\in D\setminus\{x_*\}$, estimate the
Shapley difference $(s_i - s_*)$ up to $(\frac{\epsilon}{C_\epsilon},\frac{\delta}{C_\delta})$.
Then, the Shapley value of data point $x_i$, i.e.,
$s_i$, can be estimated as $s_* + (s_i - s_*)$.
With a $(\frac{(C_\epsilon-1)\epsilon}{C_\epsilon},\frac{(C_\delta-1)\delta}{C_\delta})$-approximation for $s_*$
and a $(\frac{\epsilon}{C_\epsilon},\frac{\delta}{C_\delta})$-approximation for $(s_i - s_*)$, 
we achieve an $(\epsilon,\delta)$-approximation for $s_i$. As proved in Appendix~\ref{app:theorem_gt}, the number of model evaluations needed for estimating $N-1$ Shapley differences up to $M_1 = (\frac{\epsilon}{C_\epsilon},\frac{\delta}{C_\delta})$ is $\frac{4}{(1-q_{tot}^2)h\big(\frac{2\epsilon}{ZrC_{\epsilon}(1-q_{tot}^2)}\big)} \log \frac{C_{\delta}(N-1)}{2\delta}$. The number of model evaluations for estimating the baseline point up to $(\frac{(C_\epsilon-1)\epsilon}{C_\epsilon},\frac{(C_\delta-1)\delta}{C_\delta})$ is $M_2=\frac{4r^2C_\epsilon^2}{(C_\epsilon-1)^2\epsilon^2} \log \frac{2C_\delta}{(C_\delta-1)\delta}$. $C_\epsilon,C_\delta$ are chosen so that $M_1+M_2$ are minimized.

\paragraph*{Approach 2: Feasibility-based Approach}

An alternative approach is to solve a feasibility 
problem to recover the Shapley value for
all data points given their pairwise difference. 
In practice, this approach is less efficient as
it requires to store all pairwise ${N\choose 2}$
Shapley differences,
while the baseline point-based approach only
needs to access $N-1$ Shapley differences. In addition, this approach may require more model evaluations than the baseline point-based approach with optimized $C_\epsilon,C_\delta$. However,
we believe that it is of
theoretical interest nevertheless, as it does not require tuning $C_\epsilon$ and $C_\delta$. In this approach, we choose the number of tests as $T_f =\frac{4}{(1-q_{tot}^2)h\big(\frac{2\epsilon}{Zr(1-q_{tot}^2)}\big)} \log \frac{N(N-1)}{2\delta}$. Following a similar proof to Theorem~\ref{thm:gt_T}, we know that $C_{i,j}$ in Algorithm~\ref{alg:gt} with $T_f$ number of tests can approximate the Shapley difference between all pairs of $N$ data points up to $(\epsilon,\delta)$.
% as it gives a tighter 
% bound on the number of samples we need (it requires an
% $\epsilon$-approximation of the Shapley differences
% while the baseline point-based approach requires a
% $(c-1)\epsilon/c$-approximation of Shapley differences).

The following lemma presents the feasibility problem that can derive $(\epsilon,\delta)$-approximate Shapley values from $(\epsilon,\delta)$-approximate pairwise Shapley differences.
% with high-probability bound on the error.
% The goal is to calculate $\epsilon$-approximate Shapely differences from the test results with high-probability bound on the error. Furthermore, an approximation to the Shapley value can be derived from Shapely differences using Lemma~\ref{lm:feasibility}:

\begin{Lem}
\label{lm:feasibility}
Suppose that $C_{ij}$ is an $\epsilon$-approximation to $s_i-s_j$. Then, the solution to the feasibility problem 
    \begin{align}
        &\sum_{i=1}^N\hat{s}_i = U_{tot}\\
        \label{eqn:bound_shap_diff_1}
        &|(\hat{s}_i-\hat{s}_j)-C_{i,j}|\leq \epsilon \quad \forall i,j\in \{1,\cdots,N\}
    \end{align}
is an $\epsilon$-approximation to $s$.
\end{Lem}


\begin{proof}
Since $\sum_{i=1}^Ns_i = U_{tot}$ and $\sum_{i=1}^N\hat{s}_i = U_{tot}$, we have
\begin{align}
\label{eqn:zero_diff}
    \sum_{i=1}^N \hat{s}_i- s_i= 0
\end{align}
We prove this theorem via contradiction. Assume that $\hat{s}_i - s_i = c\epsilon$ where $c>1$. Then, by (\ref{eqn:zero_diff}), we have
\begin{align}
\label{eqn:contra}
    \sum_{j\neq i} \hat{s}_j - s_j = -c\epsilon
\end{align}
The inequalities (\ref{eqn:bound_shap_diff_1}) and (\ref{eqn:contra}) imply that
\begin{align}
    |(s_i-s_j)-C_{i,j}| + |(\hat{s}_i-\hat{s}_j)-C_{i,j}|\leq 2\epsilon
\end{align}
which gives
\begin{align}
    |(\hat{s}_i-s_i) + (s_j-\hat{s}_j)|\leq 2\epsilon
\end{align}
Under the assumption that $\hat{s}_i - s_i = c\epsilon$, we have
\begin{align}
 (-2-c)\epsilon   \leq s_j-\hat{s}_j \leq (2-c)\epsilon
\end{align}
or equivalently,
\begin{align}
\hat{s}_j - s_j \geq (c-2)\epsilon >  -\epsilon > -c\epsilon 
\end{align}
for all $j\neq i$. Thus, $\sum_{j\neq i} \hat{s}_j-s_j> -c\epsilon$, which contradicts with (\ref{eqn:contra}). 

The contradiction can be similarly established for $s_i-\hat{s}_i = c\epsilon$. Therefore, for all $i\in\{1,\cdots,N\}$, $|\hat{s}_i-s_i|\leq \epsilon$
% (c+2)\epsilon   \geq 

\end{proof}

